EgoWAM: World Action Models Beyond Pixels with In-the-Wild Egocentric Human Data

Egocentric human data offers scalable supervision for robot manipulation. However, behavior cloning entangles transferable content like objects, scenes, and task semantics, with non-transferable factors like human morphology, head motion, and behavioral style. We study whether World Action Models (WAMs) provide a better training signal by requiring policies to predict not only actions, but also how the scene evolves. The central question is what world representation best enables human-to-robot transfer. We hypothesize that an effective world target should abstract appearance, capture agent-invariant physical effects, and separate camera motion from environment change. We introduce EgoWAM, a controlled human-robot co-training framework that fixes the policy backbone, action head, and data mixture while varying only the world prediction target, comparing Pixel, DINO, and 3D motion flow. Across three real-world bimanual tasks, WAM co-training scales more effectively with in-the-wild egocentric human data than behavior cloning. Pixel-based prediction transfers weakly, while DINO and 3D flow yield substantial gains: DINO improves out-of-distribution object and scene generalization by up to 4x, and 3D flow improves in-domain performance by 20-30%. More details: https://gatech-rl2.github.io/egowam.github.io

==> figtex/exp_ablation_human_modality.tex <==
\begin{wrapfigure}{r}{0.50\textwidth}
\vspace{-40pt}
\centering
\includegraphics[width=\linewidth]{figures/exp_ablation_human_modality.pdf}

\vspace{-10pt}
\caption{\small \textbf{Ablation of Co-Train Human Data Modality.} }
\label{fig:exp-ablation-human-modality}
\vspace{-10pt}

\end{wrapfigure}

==> figtex/exp_obj.tex <==
\begin{wrapfigure}{r}{0.60\textwidth}
\vspace{-10pt}
\centering
\includegraphics[width=\linewidth]{figures/exp_obj.pdf}
\vspace{-18pt}
\caption{\small 
\textbf{In-Domain and OOD Objects.} 
}
\label{fig:exp-obj-set}
\vspace{-10pt}
\end{wrapfigure}

==> figtex/failure_pt.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/failure_pt.pdf}
    \vspace{-18pt}
    \caption{\small
    \textbf{Video Prediction for Failure Analysis on Bag-Grocery.}
    6-step rollouts from the same initial frame. \textbf{Pixel + robot only}: blurry but faithful, where the bag stays closed until acted on. \textbf{Pixel-PT + robot only}: hallucinates an already-open bag, causing the policy to skip the opening stage. \textbf{Pixel-PT + Egoverse}: sharp and faithful, showing human co-training removes the hallucination.
    }
    \label{fig:failure-pt}
\end{figure}

==> figtex/pixel_pt_dense.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/pixel_pt_dense.pdf}
  \vspace{-16pt}
  \caption{\small
  \textbf{Temporally Dense Pixel Prediction on Cup-on-Saucer.}
  Pixel-PT predicts a single future frame; Pixel-PT-Dense predicts five evenly spaced future frames over the same horizon. Both are trained on robot data only and with EgoVerse co-training. Error bars: 95\% confidence intervals ($\pm 1.96$ standard errors).
  }
  \label{fig:exp-pixel-pt-dense}
\end{figure}


==> figtex/supp_exp_setup.tex <==
\begin{figure*}[!h]
    \centering
    \includegraphics[width=\linewidth]{figures/exp_setup.pdf}
    \vspace{-16pt}
    \caption{\small
    \textbf{Robot Platform and Data Collection.}
    \textbf{(a)} Our robot platform: two upright-mounted 6-DoF ARX5 arms with two wrist-mounted Intel RealSense D405 cameras and a head-mounted Project Aria headset, teleoperated by a human via a Meta Quest 3 interface.
    \textbf{(b)} A human wearing Project Aria glasses collects demonstrations naturally.
    \textbf{(c)} The human deliberately aligns with the robot's action, height, and viewpoint, producing a static egocentric view matched to the robot platform.
    }
    \label{fig:exp-setup}
    \vspace{-12pt}
\end{figure*}

==> tables/data_composition.tex <==
\begin{table}[h]
\centering
\caption{Data composition per task. \textit{In-Domain} denotes small-scale, scene- and object-aligned human data; \textit{EgoVerse} denotes the large-scale EgoVerse-A flagship split.}
\label{tab:data_composition}
\begin{tabular}{lccc}
\toprule
\textbf{Task} & \textbf{Robot} & \textbf{Human (In-Domain)} & \textbf{Human (EgoVerse)} \\
              & (\# demos / hours) & (hours) & (hours) \\
\midrule
cup-on-saucer  & 300 / 2.5h  & 2h  & 20.5h  \\
fold-clothes   & 360 / 3.0h  & 2h  & 21h  \\
bag-grocery    & 300 / 2.5h  & 2h  & 7h  \\
\bottomrule
\end{tabular}
\end{table}

==> tables/flow_loss_modality.tex <==
\begin{table}[h]
\centering
\caption{3D-flow world-model prediction loss. Adding action labels (\textit{Action + Flow}, full \egowam) lowers the loss over \textit{Flow-Only} on both streams, supporting \emph{action as context}.}
\label{tab:flow_loss_modality}
\begin{tabular}{lcc}
\toprule
\textbf{Flow stream} & \textbf{Flow-Only} & \textbf{Action + Flow} \\
\midrule
Human & $0.23$ & $\mathbf{0.22}$ \\
Robot & $0.20$ & $\mathbf{0.19}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/model_parameters.tex <==
\begin{table}[t]
\centering
\caption{Hyperparameters held fixed across all world-model variants. Only the world-model head and target (bottom block) change between runs.}
\label{tab:model-parameters}
\small
\begin{tabular}{ll}
\toprule
\textbf{Component / Setting} & \textbf{Value} \\
\midrule
\multicolumn{2}{l}{\textit{Backbone and stems}} \\
Trunk (embed dim / blocks / heads) & $256 / 16 / 8$ \\
Query tokens consumed by trunk & $64$ action $+$ $16$ future (WAM); $64$ action only (BC) \\
Ego / wrist vision stem & ResNet-18~\cite{he2016resnet}, output dim $256$ \\
Proprioception stem & MLP ($14 \rightarrow 256$) \\
Cross-attn stem (latent / heads / head dim) & $16 / 8 / 64$ \\
Observation horizon & $1$ \\
Stochastic depth (drop path) & $0.1$ \\
\midrule
\multicolumn{2}{l}{\textit{Action head}} \\
Architecture & CrossTransformer (flow matching) \\
Blocks / hidden dim / heads & $6 / 128 / 4$ \\
Action dim $d_a$ & $14$ (per-arm 6-DoF $\mathrm{SE}(3)$ $+$ gripper) \\
Resampled chunk length $k$ & $100$ \\
Robot / human window $T_R, T_H$ & $1.5$\,s ($45$ frames) / $1.0$\,s ($30$ frames) \\
Prediction type / sampling steps & $v$-prediction / $50$ \\
Flow-matching $\tau$ prior & $\mathrm{Beta}(1.5, 1.0)$ \\
Normalization & quantile (1st/99th pct.\ $\rightarrow [-1, 1]$) \\
Deployment inference rate & $30$\,Hz \\
\midrule
\multicolumn{2}{l}{\textit{Optimization}} \\
Optimizer & AdamW (lr $1{\times}10^{-4}$, weight decay $1{\times}10^{-4}$) \\
Scheduler & cosine annealing ($T_{\max} = 1400$, $\eta_{\min} = 1{\times}10^{-5}$) \\
Batch size (robot / human) & $32 / 32$ \\
Steps per epoch / max epochs & $100 / 2000$ \\
Precision & bf16 \\
World-model loss weight $\lambda$ & $1.0$ \\
Augmentation (train only) & color jitter $(0.1, 0.1, 0.1, 0.05)$ \\
Image preprocessing & ImageNet normalization \\
\midrule
\multicolumn{2}{l}{\textit{World-model heads (swappable)}} \\
\textbf{Pixel:} VAE / decoder & Wan VAE~\cite{wan2025} / DiT, from scratch \\
\quad decoder (blocks / dim / heads) & $6 / 384 / 6$ \\
\quad latent ($C{\times}H{\times}W$) / input res & $16{\times}16{\times}16$ / $128$ \\
\textbf{Pixel-PT:} VAE / decoder & Wan VAE~\cite{wan2025} / VACE-1.3B~\cite{jiang2025vace}, pretrained \\
\quad decoder (layers / dim / heads / FFN) & $30 / 1536 / 12 / 8960$ \\
\quad latent ($C{\times}H{\times}W$) / input res & $16{\times}16{\times}16$ / $128$ \\
\textbf{DINO:} encoder / pre-processing & DINOv2-B~\cite{oquab2023dinov2}, frozen / drop {\tt[CLS]} \& registers, per-token LN \\
\quad denoiser ($\text{DiT}^{\text{DH}}$~\cite{zheng2025diffusiontransformersrepresentationautoencoders}) & DiT backbone $+$ wide DDT-style head~\cite{wang2025ddt} \\
\quad backbone (blocks / dim / heads) & $6 / 384 / 6$ \\
\quad wide head (blocks / dim) & $2 / 2048$ \\
\quad feature dim ($C{\times}H{\times}W$) & $768 {\times} 16 {\times} 16$ \\
\textbf{3D Flow:} tracker / denoiser & Track4World~\cite{lu2026track4world} / flow matching \\
\quad denoiser (blocks / dim / heads) & $4 / 256 / 4$ \\
\quad anchor grid / dim / horizon & $28{\times}40$ ($1120$ pts, no subsampling) / $3$ / $100$ \\
\quad query condition & anchor positions $q$ from current ego frame \\
\bottomrule
\end{tabular}
\end{table}
